Enhancing the Performance of Automated Grade Prediction in MOOC using Graph Representation Learning

In recent years, Massive Open Online Courses (MOOCs) have gained significant traction as a rapidly growing phenomenon in online learning. Unlike traditional classrooms, MOOCs offer a unique opportunity to cater to a diverse audience from different backgrounds and geographical locations. Renowned universities and MOOC-specific providers, such as Coursera, offer MOOC courses on various subjects. Automated assessment tasks like grade and early dropout predictions are necessary due to the high enrollment and limited direct interaction between teachers and learners. However, current automated assessment approaches overlook the structural links between different entities involved in the downstream tasks, such as the students and courses. Our hypothesis suggests that these structural relationships, manifested through an interaction graph, contain valuable information that can enhance the performance of the task at hand. To validate this, we construct a unique knowledge graph for a large MOOC dataset, which will be publicly available to the research community. Furthermore, we utilize graph embedding techniques to extract latent structural information encoded in the interactions between entities in the dataset. These techniques do not require ground truth labels and can be utilized for various tasks. Finally, by combining entity-specific features, behavioral features, and extracted structural features, we enhance the performance of predictive machine learning models in student assignment grade prediction. Our experiments demonstrate that structural features can significantly improve the predictive performance of downstream assessment tasks. The code and data are available in \url{https://github.com/DSAatUSU/MOOPer_grade_prediction}

==> related_work2.tex <==
\section{Related Work}
\label{sec:related}

Educational data mining is an emerging field that leverages computational approaches to analyze large-scale educational data~\cite{karimi2020deep,karimi2020online,karimi2019roadmap,karimi2020towards,karimi2022teachers,knake2021educational,karimi2021automatic}. In particular, computational techniques for performance prediction in MOOCs were developed over the past ten years as MOOCs gained popularity. In~\cite{ren2016predicting}, the authors developed a personalized linear multiple regression model to predict a student's future performance for specific assessment activities within a MOOC. They extracted six types of features (session features, quiz-related features, video-related features, homework-related features, time-related features, and interval-based features) from MOOC server logs to identify learning behavior and study habits for different students. Ramesh et al.~\cite{ramesh2013modeling} developed two distinct probabilistic soft logic models to forecast student achievement. One model used behavioral, linguistic, and structural features, while the other treated learner engagement as a latent variable and linked observed features to one or more types of engagement. In ~\cite{xu2016motivation}, the authors first classified learners according to motivation into three groups: \emph{certification earning}, \emph{video watching}, and \emph{course sampling}. They then used an SVM-based model to predict grades by classifying certification learners into two classes (may or may not obtain a certification). Brinton and Chiang~\cite{brinton2015mooc} applied standard algorithms to predict whether a MOOC student would be Correct on First Attempt (CFA) in answering a question. They found that parsing click-stream data into summary quantities was useful for classifying CFA. They computed nine video-watching summary quantities, such as fraction spent, fraction completed, fraction played, number of pauses, fraction paused, average playback rate, standard deviation of playback rate, number of rewinds, and number of fast forwards. Robust CFA prediction provided insights into student learning and helped instructors address students collectively. A continuous assessment prediction problem could be viewed as knowledge tracing, which predicted student's future performance based on their past activity. In~\cite{yang2017behavior}, a time series neural network was trained using lecture video watching click-streams for predicting student grades in MOOCs. Piech et al.~\cite{piech2015deep} applied RNN and LSTM networks to predict students' responses to exercises based on their past activity in MOOCs.
Furthermore, \cite{qi2018temporal} used LSTM, RNN, LR, and SVM to make individual grade predictions, with LSTM achieving the best performance with an average AUC score of 0.748. Some researchers proposed novel deep learning models to improve MOOC learner performance prediction.
In~\cite{qi2018temporal}, the authors developed a unified model that incorporated student demographics, forum activities, and learning behavior to predict students' assignment grades. They cast the prediction task as a binary classification problem, predicting whether the student's grade was ranked in the top 30\% of all students.
Kim et al.~\cite{kim2018gritnet} used deep learning methods to predict real-time student performance. They proposed a new deep learning-based method (GritNet), built upon the bidirectional long short-term memory (BLSTM) to predict student performance, such as graduation prediction. The algorithm significantly improved prediction quality within the first few weeks of the student experience. In~\cite{karimi2020online}, the authors introduced Deep Online Performance Evaluation (DOPE) to predict a student's performance in a specific course. Their method first represented the online learning system as a knowledge graph and learned student and course embeddings from historical data using a relational graph neural network. Additionally, DOPE used an LSTM to harness student behavior data into a condensed encoding since the data naturally took on a sequential shape. In~\cite{li2020peer}, the authors introduced a model using Graph Neural Networks called \begin{math}R^2GCN\end{math} (GNNs). They first created a network of questions and interactions among students, and then they utilized the proposed model to predict students' performance. Specifically, they formulated the student performance prediction in interactive online question pools as a node classification problem on a large heterogeneous network consisting of questions, students, and the interactions between them, better capturing the underlying relationship between questions and students.

All the previous studies on grade prediction in MOOCs mainly focus on course-level outcomes or major assignments, but little attention is paid to predicting grades for short, small, and specific exercises, which are called \texttt{challenges} in this study. Additionally, most existing methods ignore the complex structural relationships between pertinent entities, such as students and courses. To address these limitations, this study proposes a new approach that constructs an interaction graph between students and \texttt{challenges} and leverages advanced graph representation learning techniques to extract salient and dense entity-level vector representations. The effectiveness of this approach is validated through machine learning prediction models and extensive experiments on a new MOOC dataset introduced in this study.

% Computational techniques that target performance prediction in MOOCs have been developed during the past ten years as MOOCs have grown in popularity.


% % \textbf{Linear regression:}\ 
% The authors of ~\cite{ren2016predicting} develop a personalized linear multiple regression model to predict a student's future performance for a certain assessment activity within a MOOC. They extract 6 types of features (session features, quiz related features, video related features, homework related features, time related features and interval-based features) from the server logs of MOOCs to identify the learning behavior and study habits for different students.


% % \textbf{Probabilistic model:}\
% The authors of ~\cite{ramesh2013modeling} develop two distinct probabilistic soft logic models to forecast student achievement. One is a basic model that makes use of behavioral, linguistic, and structural features; the other is a model that treats learner engagement as a latent variable and links the various observed features to one or more types of engagement.


% % \textbf{Support vector machine:}\ 
% In ~\cite{xu2016motivation}, they first classify learners according to motivation into three groups including \emph{certification earning}, \emph{video watching} and \emph{course sampling}. Afterwards, they use a SVM-based model to make grade prediction by classifying all certification learners into two classes (may or may not obtain a certification).


% Brinton and Chiang ~\cite{brinton2015mooc} applied some standard algorithms to predict whether a MOOC student will be Correct on First Attempt (CFA) in answering a question. They saw that it is useful to parse the click-stream data into summary quantities in classifying CFA. They computed 9 video-watching summary quantities: fraction spent, fraction completed, fraction played, number of pauses, fraction paused, average playback rate, standard deviation of playback rate, number of rewinds and number of fast forwards. Robust CFA prediction can give keen insight into student learning and cluster students for the instructor to address them collectively.


% % \textbf{Deep learning:}
% A continuous assessment prediction problem can be seen as knowledge tracing which predicts student's future performance based on their past activity.
% In ~\cite{yang2017behavior}, a time series neural network was trained by using lecture video watching click-streams for predicting student grades in MOOCs. ~\cite{piech2015deep} applied RNN and LSTM networks to predict students' responses to exercises based on their past activity in MOOCs.
% More deeply, ~\cite{qi2018temporal} used LSTM, RNN, LR and SVM to make grade prediction for individuals, where LSTM achieved the best performance with an average AUC score of 0.748.

% Some research propose novel deep learning models to improve MOOCs learners' performance prediction.
% In ~\cite{qi2018temporal}, the authors develop a unified model by incorporating student demographics, forum activities and learning behavior to predict students' grades on assignments. They cast the prediction task as a binary classification problem, e.g., predicting whether the student's grade is ranked top 30\% of all students.
% Kim et al.~\cite{kim2018gritnet} use deep learning methods to achieve predicting real-time student performance. In ~\cite{kim2018gritnet}, they propose a new deep learning based method (GritNet) which builds upon the bidirectional long short term memory (BLSTM) to predict students' performance, such as graduation prediction. In fact the algorithm is able to achieve significant prediction-quality improvements within the first few weeks of the student experience.


% % \textbf{Graph Neural Network(GNNs):} 
% In ~\cite{karimi2020online}, To predict a student's performance in a particular course, they introduced Deep Online Performance Evaluation (DOPE). In order to learn student and course embeddings from historical data using a relational graph neural network, their method first represented the online learning system as a knowledge graph. In addition, DOPE used an LSTM to harness student behavior data into a condensed encoding because the data naturally takes on a sequential shape.
% In ~\cite{li2020peer}, the authors introduced a model using Graph Neural Networks called \begin{math}R^2GCN\end{math} (GNNs). They first created a network of questions and interactions amongst students, and then they utilized the suggested model to predict students' performance. In particular, they formulated the student performance prediction in interactive online question pools as a node classification problem on a large heterogeneous network consisting of questions, students, and the interactions between them, better capturing the underlying relationship between questions and students.

% \textcolor{red}{All these previous studies on grade prediction in MOOCs mainly focus on course-level outcomes or major assignments, but little attention has been paid to predicting grades for short, small, and specific exercises, which are called challenges in this study. Additionally, existing methods ignore the complex structural relationships between pertinent entities, such as students and courses. To address these limitations, this study proposes a new approach that constructs an interaction graph between students and challenges and leverages advanced graph representation learning techniques to extract salient and dense entity-level vector representations. The effectiveness of this approach is validated through machine learning prediction models and extensive experiments on a new MOOC dataset introduced in this study.}
